The GraphTempo Framework for Exploring the Evolution of a Graph through Pattern Aggregation

When the focus is on the relationships or interactions between entities, graphs offer an intuitive model for many real-world data. Such graphs are usually large and change over time, thus, requiring models and strategies that explore their evolution. We study the evolution of aggregated graphs and introduce the GraphTempo model that allows temporal and attribute aggregation not only on node level by grouping individual nodes, but on a pattern level as well, where subgraphs are grouped together. Furthermore, We propose an efficient strategy for exploring the evolution of the graph based on identifying time intervals of significant growth, shrinkage or stability. Finally, we evaluate the efficiency and effectiveness of the proposed approach using three real graphs.

==> sec3_5.tex <==
\section{Exploration}
Our goal is to use the idea of the evolution graph so as to detect interesting events in the behavior of the graph. We want to study the evolution of a graph in time intervals of different length, for example, find events that occur between two months, six months or two years, etc, and discern between three event types: \textit{growth},  \textit{shrinkage} and \textit{stability} that concern the addition, deletion and persistence respectively, of entities, nodes or edges, in the graph. %We define our problem as: \textit{detect pairs of intervals between which many events have occurred}. 

\subsection{Union and Intersection Semantics}
We are interested on changes on aggregate graphs, and as the number of aggregate graphs defined on different intervals one has to study is exponential, we need a way to efficiently explore the corresponding search space. Based on our problem definition, we are interested in considering time intervals of various lengths and not sets of intervals, thus, we require combining successive intervals to derive intervals of greater length.

Let $\mathcal{T}_i, 1\leq i\leq n$, be the intervals with shortest length. If we consider $\mathcal{T}_i$ as the elements of a set $\mathcal{T}$, we may construct the lattice of the powerset $\mathcal{T}$. Since we want to extend intervals based on combining successive intervals, we only focus on a sub lattice of the powerset lattice of $\mathcal{T}$, that is the tree that combines at each level $t$ of the lattice two elements of the previous level $t-1$ if they differ only by one element. %(Fig. \ref{fig:latt}). 
As a powerset lattice is defined on union and intersection set operators, it follows by the definitions of the temporal operators union and intersection, that the graphs defined on the time intervals of the sub lattice also form a sub lattice with respect to these operations. 

 Therefore, we can define a temporal graph using either \textit{union} semantics by considering the respective union semi-lattice, or \textit{intersection} semantics by considering the respective intersection semi-lattice. The first approach adopts a more relaxed view, where the graph defined on a union of time intervals contains all entities that exist in any of the two original time intervals. On the other hand, using intersection semantics, we adopt a stricter view, in which the intersection graph contains only entities that exist in both the original time intervals.

 

\begin{definition}[Monotonically Increasing]
We define aggregation as monotonically increasing or increasing w.r.t. a temporal operator $(\cdot)$, if given intervals $\mathcal{T}_k, \mathcal{T}_i, \mathcal{T}_j$ such that $\mathcal{T}_i \subseteq \mathcal{T}_j$ and aggregate graphs $G_i(V_i,E_i, W_{V_i}, W_{E_i}, A)$ and $G_j(V_j,E_j, W_{V_j}, W_{E_j}), A$ defined on $\mathcal{T}_k \cdot \mathcal{T}_i$ and $\mathcal{T}_k \cdot \mathcal{T}_j$ respectively, it holds that (i) $\forall v \in V_j$, if $v \in V_i$ then $w_{V_i}(v) \leq w_{V_j}(v)$, and  (ii) $\forall e \in E_j$, if $e \in E_i$ then $w_{E_i}(e) \leq w_{E_j}(e)$.
\end{definition}

\begin{definition}[Monotonically Decreasing]
We define aggregation as monotonically decreasing or decreasing w.r.t. a temporal operator $(\cdot)$, if given intervals $\mathcal{T}_k, \mathcal{T}_i, \mathcal{T}_j$ such that $\mathcal{T}_i \subseteq \mathcal{T}_j$, and aggregate graphs $G_i(V_i,E_i, W_{V_i},$ $W_{E_i}, A)$, $G_j(V_j,E_j,W_{V_j},$ $W_{E_j}, A)$ defined on $\mathcal{T}_k \cdot \mathcal{T}_i$ and $\mathcal{T}_k \cdot \mathcal{T}_j$ respectively, it holds that (i) $\forall v \in V_j$, if $v \in V_i$ then $w_{V_i}(v) \geq w_{V_j}(v)$, and  (ii) $\forall e \in E_j$, if $e \in E_i$ then $w_{E_i}(e) \geq w_{E_j}(e)$.
\end{definition}


Regarding union and intersection semantics it easily follows from their definition that:
\begin{lemma}
Aggregation is monotonically increasing with respect to union and monotonically decreasing with respect to intersection.
\end{lemma}

As union is monotonically increasing, it follows that expanding intervals using union will increase the size of the aggregate graphs and the number of events we find. Thus, the highest number of events of interest would be detected when considering the largest intervals. Consequently, in this case it is interesting to detect the minimal interval pairs at which at least $k$ events occur.
\begin{definition}[Minimal Interval Pair]
A minimal interval pair $\mathcal{T}_i, \mathcal{T}_j$ for a given threshold $k$ is defined as a pair of intervals for which at least $k$ events occurred from $\mathcal{T}_i$ to $\mathcal{T}_j$, if $\mathcal{T}_i$ precedes $\mathcal{T}_j$, or from $\mathcal{T}_j$ to $\mathcal{T}_i$ if $\mathcal{T}_j$ precedes $\mathcal{T}_i$ and for the same $\mathcal{T}_i, \nexists \mathcal{T}_{j'} \subset \mathcal{T}_j$ such that at least $k$ events occurred from $\mathcal{T}_i$ to $\mathcal{T}_{j'}$ or $\mathcal{T}_{j'}$ to $\mathcal{T}_i$ respectively.
\end{definition}


 On the other hand, as intersection is  monotonically decreasing, it follows that expanding intervals using intersection will reduce the size of the aggregate graphs and the number of events we find. Therefore, the highest number of events of interest would be detected when considering the smallest intervals. Consequently, in this case it is interesting to detect the maximal interval pairs at which at least $k$ events occur.
\begin{definition}[Maximal Interval Pair]
A maximal interval pair $\mathcal{T}_i, \mathcal{T}_j$ for a given threshold $k$ is defined as a pair of intervals for which at least $k$ events occurred from $\mathcal{T}_i$ to $\mathcal{T}_j$, if $\mathcal{T}_i$ precedes $\mathcal{T}_j$, or from $\mathcal{T}_j$ to $\mathcal{T}_i$ if $\mathcal{T}_j$ precedes $\mathcal{T}_i$, and for the same $\mathcal{T}_i, \nexists \mathcal{T}_{j'}: \mathcal{T}_j \subset \mathcal{T}_{j'}$ for which at least $k$ events occurred from $\mathcal{T}_i$ to $\mathcal{T}_{j'}$, or $\mathcal{T}_{j'}$ to $\mathcal{T}_i$ respectively.
\end{definition} 

Based on the above, we define our problem as follows.
\begin{definition}[Problem Definition]
Given an attributed graph $G$ and a time period $\mathcal{T}$ and a user-defined threshold $k$, find the minimal and maximal interval pairs in which at least $k$ events of either stability, growth or shrinkage occur.
\end{definition}


%%We propose navigating the intervals lattice for each of the three events from bottom to top so as to determine the minimal interval pairs with respect to $k$. As we have mentioned above, we can form layer $t$ of the lattice, by either extending the left or the right end of the interval of layer $t-1$.

\subsection{Stability}
Let us focus on the stability issue first. To determine the minimal or maximal interval pairs on which at least $k$ entities remain stable, we need to consider all possible pairs of intervals using union or intersection semantics respectively. We propose a more efficient exploration of the candidate interval pairs by exploiting their  monotonicity properties. 

Therefore, given two time intervals $\mathcal{T}_{old}$ and $\mathcal{T}_{new}$, where $\mathcal{T}_{old}$ precedes $\mathcal{T}_{new}$, we study stability by studying the aggregate graph $G_{\cap}$ defined on  $\mathcal{T}_{old}$, $\mathcal{T}_{new}$. We propose keeping one of the two ends of the interval fixed, as a time point of reference, and gradually extending the other end of the interval by exploiting the union or the intersection semi-lattice respectively. When our focus is on the original graph then we maintain $\mathcal{T}_{old}$ fixed as our reference point, while when our focus is on the latest state of the graph, $\mathcal{T}_{new}$ is viewed as our fixed reference point. 

We denote as $result(G)$ the number of events of interest that belong in the aggregate graph. We first consider union semantics, thus, our problem is defined as finding the minimal interval pairs in which at least $k$ entities remain stable. 

%As we study stability, the temporal operator used is intersection, i.e., we have to apply $\mathcal{T}_{old}$ \cap $\mathcal{T}_{new}$. 

Without loss of generality, we maintain $\mathcal{T}_{old}$ and gradually extend $\mathcal{T}_{new}$. 
Given $\mathcal{T}_i, 1\leq i\leq n$,  we apply the following steps:  
\begin{enumerate}
    \item First compute the aggregate graphs for all pairs $\mathcal{T}_i \cap \mathcal{T}_{i+1}$, $1\leq i<n$.
    \item If for any aggregate graph $G$ defined on $\mathcal{T}_i \cap \mathcal{T}_{i+1}$, it holds that $result(G)\geq k$, return $G$ on $\mathcal{T}_i \cap \mathcal{T}_{i+1}$ and prune any pair with $\mathcal{T}_i$ as its left end,
    \item For each pair  $\mathcal{T}_i \cap \mathcal{T}_{i+1}$ that continues, extend its right end by substituting $\mathcal{T}_{i+1}$ with its right child in the union semi-lattice (i.e., $\mathcal{T}_{i+1} \cup \mathcal{T}_{i+2}$), and apply step 2.
    \item The previous is repeated by extending the right end of each surviving interval with its right child in the union semi-lattice (i.e., $\mathcal{T}_{i+1} \cup \mathcal{T}_{i+2}\cup \dots \cup \mathcal{T}_{i+k}$) until either $i+k=n$ or no interval survives further.
\end{enumerate}
We refer to this algorithm as \textit{Union Exploration, (U-Explore)}.
U-Explore can be adapted to perform extension on the left end of each interval, i.e., by maintaining $\mathcal{T}_{new}$ fixed, and extending $\mathcal{T}_{old}$. The difference is that $\mathcal{T}_{old}$ is substituted in the next step by its left child in the union semi-lattice. 
\begin{theorem}
The minimal interval pairs for stability derived by extending $\mathcal{T}_{new}$ are not equal to those derived by extending $\mathcal{T}_{old}$. 
\end{theorem}

\begin{proof}
Let us consider of a graph consisting of $n$ $(> 2)$ time points. $T_i \cap T_{i+1}$ forms the first of our initial pairs. $T_i$ representing $T_{old}$ cannot be extended as there is no preceding time point. Therefore, w.r.t. $T_i$ as point of reference, $T_i \cap T_{i+1}$ is the only available pair. $T_{new}$, that is $T_{i+1}$ will be extended to $T_{i+1} \cup T_{i+2}, \dots, T_{i+1} \cup T_{i+2} \cup \dots \cup T_{n}$, concluding to different pairs of intervals for the same point of reference.
\end{proof}

Let us now focus on intersection semantics, thus, our problem is defined as finding the maximal intervals pairs in which at least $k$ entities (nodes or relationships) remain stable. Without loss of generality, let as assume that we maintain $\mathcal{T}_{old}$ and gradually extend $\mathcal{T}_{new}$.
Given $\mathcal{T}_i, 1\leq i\leq n$,  we apply the following steps:  
\begin{enumerate}
    \item First compute the aggregate graphs for all pairs $\mathcal{T}_i \cap \mathcal{T}_{i+1}$, $1\leq i<n$.
    \item If for any aggregate graph $G$ defined on $\mathcal{T}_i \cap \mathcal{T}_{i+1}$, it holds that $result(G)\geq k$, add $G$ to candidate set $C$, else prune  any pair with $\mathcal{T}_i$ as its left end. 
    \item For each pair  $\mathcal{T}_i \cap \mathcal{T}_{i+1}$ that continues, extend its right end by substituting $\mathcal{T}_{i+1}$ with its right child in the intersection semi-lattice (i.e., $\mathcal{T}_{i+1} \cap \mathcal{T}_{i+2}$)
    and apply step 2, and for any graph $G$ added to $C$, remove from $C$ its predecessor (i.e., the aggregate graph defined on $\mathcal{T}_i \cap \mathcal{T}_{i+1}$). 
    \item The previous is repeated by extending the right end of each surviving interval with its right child in the intersection semi-lattice (i.e., $\mathcal{T}_{i+1} \cup \mathcal{T}_{i+2}\cup \dots \cup \mathcal{T}_{i+k}$) until either $i+k=n$ or no interval survives further.
    \item The final candidate set $C$ is returned.
\end{enumerate}
We refer to this algorithm as \textit{Intersection Exploration, (I-Explore)}.
I-Explore can be adapted to perform extension on the left end of each interval, i.e., by maintaining $\mathcal{T}_{new}$ fixed, and extending $\mathcal{T}_{old}$. The difference is that $\mathcal{T}_{old}$ is substituted in the next step by its left child in the intersection semi-lattice. 


\begin{theorem}
The maximal interval pairs for stability derived by extending $\mathcal{T}_{new}$ are  equivalent to those derived by extending $\mathcal{T}_{old}$. 
\end{theorem}

\begin{proof}
Given that $T_i \cap (T_{i+1} \cap T_{i+2}) = (T_i \cap T_{i+1}) \cap T_{i+2}$ with points of reference $T_i$ and $T_{i+2}$ respectively, we derive that pairs of intervals with different points of reference give the same results if the time points participating in the pairs of intervals are identical. Therefore, extending $T_{new}$ for all initial pairs concludes to the same maximal pairs of intervals when extending $T_{old}$.
\end{proof}

\subsection{Growth}
Given two time intervals $\mathcal{T}_{old}$ and $\mathcal{T}_{new}$, where $\mathcal{T}_{old}$ precedes $\mathcal{T}_{new}$, we study growth by studying the aggregate graph of $\mathcal{T}_{new}-\mathcal{T}_{old}$, i.e., the newer graph minus the old graph to evaluate the new additions.

Let us first consider union semantics, thus, our problem is defined as finding the minimal interval pairs in which at least $k$ entities (nodes or relationships) are added. 

As difference is not a symmetric operator, our results differ when extending  $\mathcal{T}_{old}$ in contrast to  $\mathcal{T}_{new}$. When extending $\mathcal{T}_{old}$  we expect the $result(G)$ to decrease, while extending  $\mathcal{T}_{new}$ we expect causes an increase to $result(G)$. 

Let us first extend $\mathcal{T}_{old}$. We adopt U-Explore by computing at step (1), instead of the intersection, the difference graphs $\mathcal{T}_{i+1} - \mathcal{T}_i$, and then apply step (2). We claim that we do not need to proceed to further steps as  for any aggregate graph for which $result(G)<k$ extending the right interval will not increase the result size on the derived aggregate graph. 

\begin{lemma} The difference $\mathcal{T}_{new}-\mathcal{T}_{old}$ is monotonically decreasing when we extend $\mathcal{T}_{old}$ and monotonically increasing when we extend $\mathcal{T}_{new}$, using union semantics.
\label{lem:anti-union}
\end{lemma}

\begin{proof}
Let $result(G)$ the result weights of aggregate graph $G$ on $\mathcal{T}_{new}-\mathcal{T}_{old}$. Since union is monotonically increasing, for the aggregate graph on $\mathcal{T}_{old}$, $result(G_{old})$ is at most equal to the weights $result(G_{\cup old})$ for the aggregate graph defined on the union based extension of $\mathcal{T}_{old}$. 
As $result(G_{new})$ for the  aggregate graph defined on $\mathcal{T}_{new}$ remains the same, it follows that for  $result(G')$ of the aggregate graph on $\mathcal{T}_{new}-\mathcal{T}_{\cup old}$ it holds that $result(G) \leq result(G')$. Similarly, by extending $\mathcal{T}_{new}$ to $\mathcal{T}_{\cup new}$, the result of $T_{\cup new} - T_{old}$ is at least equal to $result(G)$.
\end{proof}


Let us now consider extending $\mathcal{T}_{new}$. Again, we adopt U-Explore, by computing the difference aggregate graphs $\mathcal{T}_{i+1} - \mathcal{T}_i$ instead of the intersection aggregate graphs at the respective steps. The rest of the steps are applied as defined. 

Next, we focus on intersection semantics and determine the maximal intervals pairs in which at least $k$ entities are added. We first extend $\mathcal{T}_{old}$ using intersection semantics.
\begin{lemma}
$\mathcal{T}_{new}-\mathcal{T}_{old}$ is monotonically increasing when we extend $\mathcal{T}_{old}$ and monotonically decreasing when we extend $\mathcal{T}_{new}$, using intersection semantics.
\label{lem:mon-inter}
\end{lemma}

\begin{proof}
%Similar to the proof of \label{lem:anti-union}.
Let $result(G)$ the result weights of aggregate graph $G$ on $\mathcal{T}_{new}-\mathcal{T}_{old}$. As intersection is monotonically decreasing, for the aggregate graph on $\mathcal{T}_{old}$,  $result(G_{old})$ is at least equal to the weights $result(G_{\cap old})$ for the aggregate graph defined on the intersection based extension of $\mathcal{T}_{old}$. 
As $result(G_{new})$ for the  aggregate graph defined on $\mathcal{T}_{new}$ remains the same, it follows that for  $result(G')$ of the aggregate graph on $\mathcal{T}_{new}-\mathcal{T}_{\cap old}$ it holds that $result(G) \geq result(G')$. Similarly, by extending $\mathcal{T}_{new}$ to $\mathcal{T}_{\cap new}$, the result of $T_{\cap new} - T_{old}$ is at most equal to $result(G)$.
\end{proof}

Based on the above lemma, the maximal interval pairs are: each point of reference  $\mathcal{T}_{new}$, with the longest possible $\mathcal{T}_{old}$ as long as for the defined aggregate graph, $result(G) \geq k$.

When extending $\mathcal{T}_{new}$, I-Explore is adopted appropriately. In all respective steps, we compute the aggregate difference graphs $\mathcal{T}_{i+1} - \mathcal{T}_i$, and then apply the rest of the steps accordingly.

As difference is not a symmetrical operator to exploit monotonicity properties either $\mathcal{T}_{new}$ or $\mathcal{T}_{old}$ should be extended. When we extend both $\mathcal{T}_{new}$ and $\mathcal{T}_{old}$, difference is non-monotonous irrespectively to the semantics (union or intersection) used.

\subsection{Shrinkage}
Given two time intervals $\mathcal{T}_{old}$ and $\mathcal{T}_{new}$, where $\mathcal{T}_{old}$ precedes $\mathcal{T}_{new}$, we study shrinkage based on the aggregate graph of $\mathcal{T}_{old}-\mathcal{T}_{new}$, i.e., the old graph minus the new one to evaluate deletions.

With union semantics, our problem is defined as finding the minimal intervals pairs in which at least $k$ entities (nodes or relationships) are deleted. When extending $\mathcal{T}_{old}$, we adapt U-Explore by computing  the difference graphs $\mathcal{T}_{i} - \mathcal{T}_{i+1}$. On the other hand, when extending $\mathcal{T}_{new}$, as according to lemma \ref{lem:anti-union}, the operator is monotonically decreasing, we only need to evaluate the difference aggregate graphs on pairs of the shortest intervals (i.e., step 1 of U-Explore) and check their result with respect to $k$.


With intersection semantics we determine the maximal intervals pairs in which at least $k$ entities are deleted. When extending $\mathcal{T}_{new}$, I-Explore is adapted appropriately by computing the aggregate difference graphs $\mathcal{T}_{i} - \mathcal{T}_{i+1}$. When extending $\mathcal{T}_{old}$, according to lemma \ref{lem:mon-inter} the operator is monotonically increasing and again for each reference point $\mathcal{T}_{new}$, the longest possible $\mathcal{T}_{old}$ forms the maximal interval and it suffices to check whether $result(G) \geq k$.



All cases are summarized on Table \ref{tab:expl}. Column \textit{Case} shows which is the reference point and which interval is extended using either union ($\cup$) or intersection ($\cap$) semantics. Columns \textit{Left} and \textit{Right} refer to the left and right interval in the result interval pairs. One of the elements in the pair is always a time point (t.p.) while the other can be either of type time point (t.p.) or interval and longest interval. The last column shows the relationships between the results of different cases, and in particular when the result of one case is a subset of the result of another case.

\subsection{Initialization of \textit{k}}
The appropriate value of the threshold $k$ depends each time on the given graph and its data. To configure this threshold, we propose an initial value for $k$, indicating a threshold of interestingness and acting as a starting point so as to attain some results and then continue with its tuning. In particular, given the type of entity we are interested in, we initialize $k$ to a value $w_{th}$ which is defined as the minimum or the maximum weight of the given type of entity in the aggregation graph for any graph defined on the temporal aggregation of pairs of consecutive time points. For stability, we compute the aggregate graphs on intersections of pairs of consecutive time points, while for growth and shrinkage we compute the aggregate graphs on the appropriate difference graphs. Further, for a monotonically increasing operator, we start with  $w_{th}$ as the minimum aggregation weight for a given entity type, and increase it gradually, while for the monotonically decreasing operators $w_{th}$ corresponds to the maximum aggregation weight and is gradually decreased as the exploration progresses.


% \begin{table*}
% %\vspace{-0.25in}
% \caption{Exploration Intervals Properties | Growth}
% \label{tab:grow}
% \centering
% \begin{tabular}{c|c|c|ccccccc}
% \hline
% \centering
% \ & & Operation & Left & Right & Monotonous & Anti-monotonous & $\subseteq$ of & Left $\subseteq$ of & Right $\subseteq$ of\\ \hline
% \ Min. & i & New (-) Old($\cup$) & t.p. & t.p. & & & ii & & iii\\
% \ & ii & New($\cup$) (-) Old & t.p. / interval & t.p. & X & & & iv\\ \hline
% \ Max. & iii & New (-) Old($\cap$) & t.p. & longest interval & X & & & \\
% \ & iv & New($\cap$) (-) Old & t.p. / interval & t.p. & & X & & \\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}
% %\vspace{-0.25in}
% \caption{Exploration Intervals Properties | Shrinkage}
% \label{tab:shrink}
% \centering
% \begin{tabular}{c|c|c|ccccccc}
% \hline
% \centering
% \ & & Operation & Left & Right & Monotonous & Anti-monotonous & $\subseteq$ of & Left $\subseteq$ of & Right $\subseteq$ of\\ \hline
% \ Min. & i & Old($\cup$) (-) New & t.p. / interval & t.p. & & & & iii & \\
% \ & ii & Old (-) New($\cup$) & t.p. & t.p. & X & & i & & iv\\ \hline
% \ Max. & iii & Old($\cap$) (-) New & t.p. / interval & t.p. & & X & & & \\
% \ & iv & Old (-) New($\cap$) & t.p. & longest interval & X & & & &\\ \hline
% \end{tabular}
% \end{table*}

% \begin{table*}
% %\vspace{-0.25in}
% \caption{Exploration Intervals Properties | Stability}
% \label{tab:stab}
% \centering
% \begin{tabular}{c|c|c|ccccccc}
% \hline
% \centering
% \ & & Operation & Left & Right & Monotonous & Anti-monotonous & $\subseteq$ of & Left $\subseteq$ of & Right $\subseteq$ of\\ \hline
% \ Min. & i & Old($\cup$) $\cap$ New & t.p. / interval & t.p. & X & & & iii & \\
% \ & ii & New($\cup$) $\cap$ Old & t.p. / interval & t.p. & X & & & iv & \\ \hline
% \ Max. & iii & Old($\cap$) $\cap$ New & t.p. / interval & t.p. & & X & & & \\
% \ & iv & New($\cap$) $\cap$ Old & t.p. / interval & t.p. & & X & & & \\ \hline
% \end{tabular}
% \end{table*}


% \begin{table*}
% %\vspace{-0.25in}
% \caption{Exploration Intervals Properties}
% \label{tab:expl}
% \setlength\tabcolsep{2pt}
% \begin{tabular}{c|c|c|ccccccc}
% \hline
% \centering
% \ Case & Type & Operation & Left & Right & Monotonous & Anti-monotonous & $\subseteq$ of & Left $\subseteq$ of & Right $\subseteq$ of\\ \hline
% \multirow{4}{*}{Growth} & \multirow{2}{*}{Min.} & New - Old($\cup$) & t.p. & t.p. & & & New($\cup$) - Old & & Old($\cap$)\\
% \ & & New($\cup$) - Old & t.p. / interval & t.p. & \checkmark & & & New($\cap$) & \\
% \ & \multirow{2}{*}{Max.} & New - Old($\cap$) & t.p. & longest interval & \checkmark & & & &\\
% \ & & New($\cap$) - Old & t.p. / interval & t.p. & & \checkmark & & & \\ \hline\hline
% \multirow{4}{*}{Shrinkage} & \multirow{2}{*}{Min.} & Old($\cup$) - New & t.p. / interval & t.p. & & & & Old($\cap$) & \\
% \ & & Old - New($\cup$) & t.p. & t.p. & \checkmark & & Old($\cup$) - New & & New($\cap$) \\
% \ & \multirow{2}{*}{Max.} & Old($\cap$) - New & t.p. / interval & t.p. & & \checkmark & & & \\
% \ & & Old - New($\cap$) & t.p. & longest interval & \checkmark & & & &\\ \hline\hline
% \multirow{4}{*}{Stability} & \multirow{2}{*}{Min.} & Old($\cup$) $\cap$ New & t.p. / interval & t.p. & \checkmark & & & Old($\cap$) & \\
% \ & & New($\cup$) $\cap$ Old & t.p. / interval & t.p. & \checkmark & & & New($\cap$) & \\
% \ & \multirow{2}{*}{Max.} & Old($\cap$) $\cap$ New & t.p. / interval & t.p. & & \checkmark & New($\cap$) $\cap$ Old & & \\
% \ & & New($\cap$) $\cap$ Old & t.p. / interval & t.p. & & \checkmark & Old($\cap$) $\cap$ New & & \\ \hline
% \end{tabular}
% \end{table*}




\begin{comment}\begin{figure}
\centering
\includegraphics[scale=0.25]{figures_examples/6.lattice.png}
%\vspace*{-0.1in}
\caption{Lattice representation.}
\label{fig:latt}
\end{figure}
\end{comment}



\begin{table*}
%\vspace{-0.25in}
\caption{Exploration Intervals Properties}
\centering
\label{tab:expl}
\setlength\tabcolsep{2pt}
\begin{tabular}{c|c|c|ccccc}
\hline
\centering
\ Event & Type & Case & Left & Right & Mon. Increasing & Mon. Decreasing & $\subseteq$ of\\ \hline
\multirow{4}{*}{Growth} & \multirow{2}{*}{Min.} & $\mathcal{T}_{new}$ - $\mathcal{T}_{old}$($\cup$) & t.p. & t.p. & & \checkmark & $\mathcal{T}_{new}$($\cup$) - $\mathcal{T}_{old}$\\
\ & & $\mathcal{T}_{new}$($\cup$) - $\mathcal{T}_{old}$ & t.p. / interval & t.p. & \checkmark & &\\
\ & \multirow{2}{*}{Max.} & $\mathcal{T}_{new}$ - $\mathcal{T}_{old}$($\cap$) & t.p. & longest interval & \checkmark & &\\
\ & & $\mathcal{T}_{new}$($\cap$) - $\mathcal{T}_{old}$ & t.p. / interval & t.p. & & \checkmark &\\ \hline\hline
\multirow{4}{*}{Shrinkage} & \multirow{2}{*}{Min.} & $\mathcal{T}_{old}$($\cup$) - $\mathcal{T}_{new}$ & t.p. / interval & t.p. & \checkmark & &\\
\ & & $\mathcal{T}_{old}$ - $\mathcal{T}_{new}$($\cup$) & t.p. & t.p. & & \checkmark & $\mathcal{T}_{old}$($\cup$) - $\mathcal{T}_{new}$\\
\ & \multirow{2}{*}{Max.} & $\mathcal{T}_{old}$($\cap$) - $\mathcal{T}_{new}$ & t.p. / interval & t.p. & & \checkmark &\\
\ & & $\mathcal{T}_{old}$ - $\mathcal{T}_{new}$($\cap$) & t.p. & longest interval & \checkmark & &\\ \hline\hline
\multirow{4}{*}{Stability} & \multirow{2}{*}{Min.} & $\mathcal{T}_{old}$($\cup$) $\cap$ $\mathcal{T}_{new}$ & t.p. / interval & t.p. & \checkmark & & \\
\ & & $\mathcal{T}_{new}$($\cup$) $\cap$ $\mathcal{T}_{old}$ & t.p. / interval & t.p. & \checkmark & &\\
\ & \multirow{2}{*}{Max.} & $\mathcal{T}_{old}$($\cap$) $\cap$ $\mathcal{T}_{new}$ & t.p. / interval & t.p. & & \checkmark & $\mathcal{T}_{new}$($\cap$) $\cap$ $\mathcal{T}_{old}$\\
\ & & $\mathcal{T}_{new}$($\cap$) $\cap$ $\mathcal{T}_{old}$ & t.p. / interval & t.p. & & \checkmark & $\mathcal{T}_{old}$($\cap$) $\cap$ $\mathcal{T}_{new}$\\ \hline
\end{tabular}
\end{table*}
